ReListen: Training-Free Evidence Localization in Hour-Long Audio with Frozen Audio Language Models

Audio language models are meant to answer questions from the audio itself, but an hour-long recording rarely fits in their context, and the answer often depends on a few seconds of it. Transcribing the recording first makes it fit but discards sounds and voices, while systems that return to the audio must be trained for this behavior. We propose ReListen, a training-free method in which a frozen audio language model finds its own evidence before answering. In a Jev-style scan, the model scores each 20-second window by the probability that it helps answer the question, and it then answers from the highest-scoring minute. This minute overlaps the annotated evidence far more often than transcript retrieval, for 88.5% of VoiceGiraffe questions. Without any change, the same scan also grounds events on LAT-Bench as well as a model trained for temporal grounding. Answering from it matches or exceeds hearing the whole recording with a small fraction of the audio, and on VoiceGiraffe it exceeds a transcript of the whole recording by 9.2 points. The selected evidence is also worth hearing rather than reading. Given the same excerpts, reading their transcript matches listening on speech content, but listening is clearly more accurate on questions about sounds and voices. Moreover, ReListen answers faster than every transcript-based system, and its memory stays constant even for recordings too long to hear whole on one GPU. Therefore, a frozen audio language model can search hour-long recordings by itself, without a transcript or additional training.

==> figures/accuracy_time_data.tex <==
\def\atLASReaderTranscriptX{119.28}\def\atLASReaderTranscriptY{59.6}
\def\atLASWhisperX{27.57}\def\atLASWhisperY{58.1}
\def\atLASEchoX{156.76}\def\atLASEchoY{58.1}
\def\atLASSpeakerX{1124.31}\def\atLASSpeakerY{53.0}
\def\atLASFullX{11.36}\def\atLASFullY{54.6}
\def\atLASReListenX{17.33}\def\atLASReListenY{53.5}
\def\atLASReListenFourX{5.56}\def\atLASReListenFourY{53.5}
\def\atLASFastX{10.02}\def\atLASFastY{53.7}
\def\atLASFastFourX{3.66}\def\atLASFastFourY{53.7}
\def\atVGReaderTranscriptX{134.95}\def\atVGReaderTranscriptY{52.8}
\def\atVGEchoX{168.64}\def\atVGEchoY{58.1}
\def\atVGSpeakerX{1047.75}\def\atVGSpeakerY{55.7}
\def\atVGFullX{11.64}\def\atVGFullY{51.4}
\def\atVGReListenX{16.98}\def\atVGReListenY{62.0}
\def\atVGReListenFourX{5.66}\def\atVGReListenFourY{62.0}
\def\atVGFastX{9.04}\def\atVGFastY{60.9}
\def\atVGFastFourX{3.60}\def\atVGFastFourY{60.9}

